Sparseloop: An Analytical Approach To Sparse Tensor Accelerator Modeling

In recent years, many accelerators have been proposed to efficiently process sparse tensor algebra applications (e.g., sparse neural networks). However, these proposals are single points in a large and diverse design space. The lack of systematic description and modeling support for these sparse tensor accelerators impedes hardware designers from efficient and effective design space exploration. This paper first presents a unified taxonomy to systematically describe the diverse sparse tensor accelerator design space. Based on the proposed taxonomy, it then introduces Sparseloop, the first fast, accurate, and flexible analytical modeling framework to enable early-stage evaluation and exploration of sparse tensor accelerators. Sparseloop comprehends a large set of architecture specifications, including various dataflows and sparse acceleration features (e.g., elimination of zero-based compute). Using these specifications, Sparseloop evaluates a design's processing speed and energy efficiency while accounting for data movement and compute incurred by the employed dataflow as well as the savings and overhead introduced by the sparse acceleration features using stochastic tensor density models. Across representative accelerators and workloads, Sparseloop achieves over 2000 times faster modeling speed than cycle-level simulations, maintains relative performance trends, and achieves 0.1% to 8% average error. With a case study, we demonstrate Sparseloop's ability to help reveal important insights for designing sparse tensor accelerators (e.g., it is important to co-design orthogonal design aspects).

==> 00_abstract.tex <==
\begin{abstract}
In recent years, many accelerators have been proposed to efficiently process sparse tensor algebra applications (\eg, sparse neural networks). However, these proposals are single points in a large and diverse design space. The lack of systematic description and modeling support for these sparse tensor accelerators impedes hardware designers from efficient and effective design space exploration.

This paper first presents a unified taxonomy to systematically describe the diverse sparse tensor accelerator design space. Based on the proposed taxonomy, it then introduces \tool, the first fast, accurate, and flexible analytical modeling framework to enable early-stage evaluation and exploration of sparse tensor accelerators. \tool~comprehends a large set of architecture specifications, including various dataflows and sparse acceleration features (\eg, elimination of zero-based compute). Using these specifications, \tool~evaluates a design's processing speed and energy efficiency while accounting for data movement and compute incurred by the employed dataflow, including the savings and overhead introduced by the sparse acceleration features using stochastic  density models.

Across representative accelerator designs and workloads, \tool~achieves over 2000$\times$ faster modeling speed than cycle-level simulations, maintains relative performance trends, and achieves 0.1\% to 8\% average error. The paper also presents example use cases of \tool~in different accelerator design flows to reveal important design insights.
% {\color{red} With the presented case studies, we demonstrate example use cases of \tool~in accelerator design flows to explore and compare different design alternatives to reveal important design insights.}

%With comparable hardware resources, accelerators studied can have up to a 5x difference in energy-delay-product.
%less than 1\% error compared to a custom accelerator model with statistical data characterization, and less than 8\% error compared to simulations with real data. 

\end{abstract}

==> Makefile <==
PDF = sample-micro52.pdf

all: ${PDF}

%.pdf: %.tex acmart.cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.gz *.zip *.rpi \
  $(PDF) *-converted-to.pdf


==> tables/fiber_based_compute_fga.tex <==
\begin{table}[tb]
\centering
\begin{tabular}{|c|c|}
 \hline
\textbf{State of Operands}     & \textbf{Possible Behaviors}                                                                       \\
 \hline
Non-Empty; Non-Empty & Actual compute                                                                           \\
 \hline
Non-Empty; Empty     & \begin{tabular}[c]{@{}c@{}}Actual compute (default)\\ Gated compute\end{tabular}                   \\
 \hline
Non-Empty; Not Exist & \begin{tabular}[c]{@{}c@{}}Actual compute (default)\\ Gated compute\\ Skipped compute\end{tabular} \\
 \hline
Empty; Empty         & \begin{tabular}[c]{@{}c@{}}Actual compute (default) \\ Gated compute\end{tabular}                   \\
 \hline
Empty; Not Exist     & \begin{tabular}[c]{@{}c@{}}Actual compute (default) \\ Gated compute\\ Skipped compute\end{tabular} \\
\hline
\end{tabular}
\caption{Example compute unit behaviors with two operands.}
\label{tab:compute_fga}
\end{table}

==> tables/fiber_based_storage_fga.tex <==
\begin{table}[]
\begin{tabular}{|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Dependent on \\ statistical fibertree  characterizations\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dependent on \\ SAFs applied\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Non-empty \\ fiber elements\end{tabular}}             & Actual accesses                                                      \\ \cline{2-2} 
                                                                                                 & Gated accesses                                                       \\ \cline{2-2} 
                                                                                                 & Skipped accesses                                                     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Empty \\ fiber elements\end{tabular}}                 & Actual accesses                                                      \\ \cline{2-2} 
                                                                                                 & Gated accesses                                                       \\ \cline{2-2} 
                                                                                                 & Skipped accesses                                                     \\ \hline
\end{tabular}
\end{table}
